Large Language Model Safety: A Holistic Survey

The rapid development and deployment of large language models (LLMs) have introduced a new frontier in artificial intelligence, marked by unprecedented capabilities in natural language understanding and generation. However, the increasing integration of these models into critical applications raises substantial safety concerns, necessitating a thorough examination of their potential risks and associated mitigation strategies. This survey provides a comprehensive overview of the current landscape of LLM safety, covering four major categories: value misalignment, robustness to adversarial attacks, misuse, and autonomous AI risks. In addition to the comprehensive review of the mitigation methodologies and evaluation resources on these four aspects, we further explore four topics related to LLM safety: the safety implications of LLM agents, the role of interpretability in enhancing LLM safety, the technology roadmaps proposed and abided by a list of AI companies and institutes for LLM safety, and AI governance aimed at LLM safety with discussions on international cooperation, policy proposals, and prospective regulatory directions. Our findings underscore the necessity for a proactive, multifaceted approach to LLM safety, emphasizing the integration of technical solutions, ethical considerations, and robust governance frameworks. This survey is intended to serve as a foundational resource for academy researchers, industry practitioners, and policymakers, offering insights into the challenges and opportunities associated with the safe integration of LLMs into society. Ultimately, it seeks to contribute to the safe and beneficial development of LLMs, aligning with the overarching goal of harnessing AI for societal advancement and well-being. A curated list of related papers has been publicly available at https://github.com/tjunlp-lab/Awesome-LLM-Safety-Papers.

==> taxonomies/Value_Misalighment_Taxonomy.tex <==
\tikzstyle{my-box}=[
    rectangle,
    draw=hidden-draw,
    rounded corners,
    text opacity=1,
    minimum height=1.5em,
    minimum width=5em,
    inner sep=2pt,
    align=center,
    fill opacity=.5,
    line width=0.8pt,
]
\tikzstyle{leaf}=[my-box, minimum height=1.5em,
    fill=hidden-pink!80, text=black, align=center,font=\normalsize,
    inner xsep=2pt,
    inner ysep=4pt,
    line width=0.8pt,
]
\begin{figure*}[t!]
    \centering
    \resizebox{\textwidth}{!}{
        \begin{forest}
            forked edges,
            for tree={
                grow=east,
                reversed=true,
                anchor=base west,
                parent anchor=east,
                child anchor=west,
                base=center,
                font=\large,
                rectangle,
                draw=hidden-draw,
                rounded corners,
                align=center,
                text centered,
                minimum width=5em,
                edge+={darkgray, line width=1pt},
                s sep=3pt,
                inner xsep=2pt,
                inner ysep=3pt,
                line width=0.8pt,
                ver/.style={rotate=90, child anchor=north, parent anchor=south, anchor=center},
            },
            where level=1{text width=10em,font=\normalsize,}{},
            where level=2{text width=13.5em,font=\normalsize,}{},
            where level=3{text width=15em,font=\normalsize,}{},
            where level=4{text width=15em,font=\normalsize,}{},
            [
                Value \\ Misalignment
                [
                   Social \\ Bias
                   [
                        Preliminaries
                        [
                            Safety Impact of Social Bias%Types of Privacy \\ Information
                            [
                            \citet{DBLP:journals/corr/BlodgettO17} \\
                            \citet{article} \\
                            \citet{DBLP:conf/emnlp/ShengCNP19} \\
                            \citet{DBLP:conf/sigir/RekabsazS20} \\
                            \citet{DBLP:conf/sigir/RekabsazKS21} \\
                            \citet{DBLP:conf/fat/BenderGMS21} \\
                            \citet{DBLP:conf/emnlp/Dev0PS21} \\
                            \citet{mechura-2022-taxonomy} \\
                            \citet{obermeyer2019dissecting} \\
                            , leaf
                            ]
                        ]
                        [
                            Social Bias in LLM lifecycle
                            [
                            \citet{DBLP:conf/aies/AbidF021} \\
                            \citet{DBLP:conf/icml/LiangWMS21} \\
                            \citet{seyyed2021underdiagnosis} \\
                            \citet{DBLP:journals/corr/abs-2309-00770} \\
                            \citet{DBLP:journals/firstmonday/Ferrara23a} \\
                            , leaf
                            ]
                        ]
                    ]
                    [
                        Mitigation \\ Methods
                        [
                            Pre-Processing Mitigation
                            [
                            \citet{DBLP:conf/aaai/ZayedPMPSC23} \\
                            \citet{DBLP:conf/acl/ChungKA23} \\
                            , leaf
                            ]
                        ]
                        [
                            Pre-Training Mitigation
                            [
                            \citet{DBLP:conf/emnlp/LauscherLG21} \\
                            \citet{DBLP:conf/ltedi/GiraZL22} \\
                            \citet{DBLP:conf/ijcnlp/GarimellaMA22} \\
                            \citet{DBLP:journals/corr/abs-2207-02463} \\
                            , leaf
                            ]
                        ]
                        [
                            Post-Training Mitigation
                            [
                            \citet{DBLP:journals/mta/LinWCS21} \\
                            \citet{DBLP:conf/aies/ZhangLM18} \\
                            \citet{DBLP:journals/npjdm/YangSEYC23} \\
                            \citet{DBLP:conf/wsdm/ParkCYK23} \\
                            \citet{DBLP:conf/www/ZafarVGG17} \\
                            \citet{DBLP:journals/corr/abs-2106-07849} \\
                            , leaf
                            ]
                        ]
                        [
                            Inference Mitigation
                            [
                            \citet{DBLP:journals/npjdm/MittermaierRK23a} \\
                            \citet{DBLP:conf/iclr/YangYLL023} \\
                            \citet{DBLP:conf/emnlp/LauscherLG21} \\
                            , leaf
                            ]
                        ]
                    ]
                    [
                        Evaluation
                        [
                            Metrics
                            [
                                \citet{caliskan2017semantics} \\
                                \citet{DBLP:conf/naacl/MayWBBR19} \\
                                \citet{panch2019artificial} \\
                                \citet{DBLP:journals/corr/abs-2010-06032} \\
                                \citet{DBLP:conf/aies/GuoC21} \\
                                , leaf
                            ]
                        ]
                        [
                            Benchmarks
                            [
                                \citet{DBLP:conf/birthday/LuMWAD20} \\
                                \citet{DBLP:conf/naacl/RudingerNLD18} \\
                                \citet{DBLP:conf/naacl/ZhaoWYOC18} \\
                                \citet{DBLP:journals/tacl/WebsterRAB18} \\
                                \citet{DBLP:conf/emnlp/NangiaVBB20} \\
                                \citet{DBLP:conf/emnlp/LiKKSS20} \\
                                \citet{DBLP:conf/fat/DhamalaSKKPCG21} \\
                                \citet{DBLP:conf/acl/BarikeriLVG20} \\
                                \citet{DBLP:conf/nodalida/HanssonMABD21} \\
                                \citet{DBLP:conf/emnlp/SmithHKPW22} \\
                                \citet{DBLP:conf/coling/HuangX24} \\
                                \citet{DBLP:conf/acl/ParrishCNPPTHB22} \\
                                , leaf
                            ]
                        ]
                   ]
                ]
            ]
        \end{forest}
    }
    \caption{Overview of Value Misalignment of LLMs.}
    \label{fig:Overview_of_value_misalignment}
\end{figure*}
